Improved Sample Complexity for Incremental Autonomous Exploration in MDPs

We investigate the exploration of an unknown environment when no reward function is provided. Building on the incremental exploration setting introduced by Lim and Auer [1], we define the objective of learning the set of $\epsilon$-optimal goal-conditioned policies attaining all states that are incrementally reachable within $L$ steps (in expectation) from a reference state $s_0$. In this paper, we introduce a novel model-based approach that interleaves discovering new states from $s_0$ and improving the accuracy of a model estimate that is used to compute goal-conditioned policies to reach newly discovered states. The resulting algorithm, DisCo, achieves a sample complexity scaling as $\tilde{O}(L^5 S_{L+\epsilon} \Gamma_{L+\epsilon} A \epsilon^{-2})$, where $A$ is the number of actions, $S_{L+\epsilon}$ is the number of states that are incrementally reachable from $s_0$ in $L+\epsilon$ steps, and $\Gamma_{L+\epsilon}$ is the branching factor of the dynamics over such states. This improves over the algorithm proposed in [1] in both $\epsilon$ and $L$ at the cost of an extra $\Gamma_{L+\epsilon}$ factor, which is small in most environments of interest. Furthermore, DisCo is the first algorithm that can return an $\epsilon/c_{\min}$-optimal policy for any cost-sensitive shortest-path problem defined on the $L$-reachable states with minimum cost $c_{\min}$. Finally, we report preliminary empirical results confirming our theoretical findings.

==> sec_comparison.tex <==

% !TEX root=MAIN_AutExp.tex

\section{OLD------Discussion} 
\label{section_comparison_discussion}
\todojout{This is mostly our old section \ref{section_comparison_discussion}. To discuss and revamp. }

\paragraph{Comparison with \UcbExplore~\cite{lim2012autonomous}.} \UcbExplore maintains a set $\mathcal{K}$ of \say{known} states and a set $\mathcal{U}$ of \say{unknown} states, and alternates between two phases of \textit{state discovery} and \textit{policy evaluation}. The core difference with \ALGO is that the policy evaluation phase is performed online, as a candidate policy is marked as successful if it displays a satisfactory \textit{empirical performance}, which is evaluated with rollouts of length $H_{\Ucb} := \lceil L + \frac{L^2}{\epsilon} \rceil$. \UcbExplore satisfies the following \DCthree sample complexity (\cite[][Thm.\,8]{lim2012autonomous}).\footnote{Note that if we replace the error of $\epsilon$ for \DCthree with an error of $L\epsilon$ as in the original paper \citep{lim2012autonomous}, we recover their stated sample complexity in $\wt{O}\left(\frac{L^3 S_{L + \epsilon} A}{\epsilon^3} \right)$.}
%\begin{proposition}[Thm.~8 of \citealp{lim2012autonomous}] 
\begin{align}
    \mathcal{C}_{\DCthree}(\UcbExplore,L,\epsilon,\delta) = \wt{O}\left(\frac{L^6 S_{L+\epsilon} A}{\epsilon^3} \right).
\label{eq_corrected_ucbexplore}
\end{align}
%\label{theorem_corrected_ucbexplore}
%\end{proposition}

While \UcbExplore succeeds in having a sample complexity depend linearly in $S_{L + \epsilon}$, its dependency in $\epsilon$ as well as $L$ is worse than \ALGO. We now provide insight as to why the bound of Eq.\,\eqref{eq_corrected_ucbexplore} inherits a $\wt{O}(\epsilon^{-3})$ dependency. The high-level explanation is that the optimistic policies computed by \UcbExplore solve a \textit{finite-horizon problem} (with the horizon set to $H_{\Ucb}$). However, minimizing the expected time to reach a target state is intrinsically an SSP problem, which is exactly what \ALGO leverages. By computing policies that solve a finite-horizon problem (note that they reset every $H_{\Ucb}$ time steps), the \UcbExplore analysis sets the horizon to $H_{\Ucb} := \lceil L + L^2 \epsilon^{-1} \rceil$, %\footnote{An intuition behind the choice of $H_{\Ucb}$ in \UcbExplore can be obtained from Markov's inequality which gives that, for any $s \in \mathcal{S}_L^{\rightarrow}$ and policy $\pi$ for which $v_{\pi}(s_0 \rightarrow s) \leq L$, we have $q_{\pi,H_{\Ucb}}(s_0 \rightarrow s) \leq \frac{v_{\pi}(s_0 \rightarrow s)}{H_{\Ucb}} \sim \epsilon$ whenever $H_{\Ucb} \sim \frac{L}{\epsilon}$.}
i.e., it regrettably scales as $\epsilon^{-1}$ and leads to a sample complexity scaling as $\wt{O}(H_{\Ucb} \epsilon^{-2}) = \wt{O}(\epsilon^{-3})$. In contrast, we prove in App.\,\ref{app_effective_horizon_problem} that the effective horizon of the problem actually only scales as $\log(\epsilon^{-1}) L$, thus inducing a $\wt{O}(\epsilon^{-2})$ sample complexity.



\todoa{TODO}
Nevertheless, \UcbExplore is unable to tackle \DCone. Indeed, the algorithm does not track the samples it collects and is thus unable to backtrack and re-compute the shortest-path policies as the set $\mathcal{K}$ grows (which corresponds to step \ding{176} in \ALGO).


As a summary, Table \ref{tab:comparison} reports the sample complexity of \ALGO and \UcbExplore. The critical distinction is that \ALGO succeeds in tackling condition \DCone while \UcbExplore fails to do so. As for the two weaker conditions \DCtwo and \DCthree which both algorithms fulfill, \ALGO yields a better dependency on $\epsilon$ and $L$ (especially for condition \DCtwo), while \UcbExplore has a better dependency on $S_{L + \epsilon}$. It remains an open and interesting question whether it is possible to design an algorithm that can tackle \DCone as well as combine attractive dependencies in $\epsilon$, $L$ and $S_{L + \epsilon}$.  


Note that the computational complexities of \ALGO and \UcbExplore are roughly equivalent. Indeed, although the sample collection phase of \ALGO is more thorough that \UcbExplore and thus more states may belong to $\mathcal{U}$, \ALGO performs computations restricted to a set of candidate states which according to Lem.\,\ref{lem:W_k} is of the same size as the set of candidate states in \UcbExplore. 

Finally, a compelling advantage of \ALGO is that it carefully designs shortest-path policies that can effectively estimate \textit{uniformly accurately} the transition probabilities of the MDP $M$ restricted to the subset of interest $\mathcal{S}_L^{\rightarrow}$. The algorithm thus does not only learn targeted navigation from $s_0$ to any state in $\mathcal{S}_L^{\rightarrow}$, but also learns a $O(\epsilon)$-induced model of $p$ restricted to $\mathcal{S}_L^{\rightarrow}$. This implies that the agent is able to leverage its fine-grained knowledge of the environment to solve other tasks. For instance, it could learn to quickly navigate between states in $\mathcal{S}_L^{\rightarrow}$ without having to perform the \RESET action, or it could learn to tackle faster a standard reinforcement learning task if a reward signal is provided. Furthermore, the agent can be \textit{robust} to changes in the problem parameters such as $L$ or $\epsilon$, in contrast to \UcbExplore which needs to restart its sample collection from scratch whenever $L$ or $\epsilon$ change. 

\todoa{Leftover}
We conclude this section by recalling that \UcbExplore~\cite{lim2012autonomous} is able to achieve \DCthree with a sample complexity scaling as\todoaout{Explain the big-O notation.} $\wt{O}_{\epsilon}( L^6 S_{L+\epsilon} A \epsilon^{-3})$. Nonetheless, \UcbExplore is unable to return $\epsilon$-optimal policies in the sense of \DCone. Interestingly, while \UcbExplore can be easily tweaked to achieve stronger guarantees than \DCthree (at the cost of an additional factor $L/\epsilon$ in the sample complexity), it never computes accurate enough estimates of the environment to be able to compute $\epsilon$-optimal shortest-path policies restricted on the whole set $\mathcal{S}_L^{\rightarrow}$ (see App.~\ref{app_objectives} for further discussion). In the next section, we introduce a simple but radically different algorithmic approach to enable such stronger result.\todoaout{This whole paragraph can be removed.}


